Deep Gaze I: Boosting Saliency Prediction with Feature Maps Trained on ImageNet

Recent results suggest that state-of-the-art saliency models perform far from optimal in predicting fixations. This lack in performance has been attributed to an inability to model the influence of high-level image features such as objects. Recent seminal advances in applying deep neural networks to tasks like object recognition suggests that they are able to capture this kind of structure. However, the enormous amount of training data necessary to train these networks makes them difficult to apply directly to saliency prediction. We present a novel way of reusing existing neural networks that have been pretrained on the task of object recognition in models of fixation prediction. Using the well-known network of Krizhevsky et al. (2012), we come up with a new saliency model that significantly outperforms all state-of-the-art models on the MIT Saliency Benchmark. We show that the structure of this network allows new insights in the psychophysics of fixation selection and potentially their neural implementation. To train our network, we build on recent work on the modeling of saliency as point processes.

==> figures/used_features/data.tex <==
\expandafter\xdef\csname used_features_ratio_9\endcsname{0.64}
\expandafter\xdef\csname used_features_ratio_8\endcsname{0.65}
\expandafter\xdef\csname used_features_ratio_7\endcsname{0.66}
\expandafter\xdef\csname used_features_ratio_6\endcsname{0.70}
\expandafter\xdef\csname used_features_ratio_5\endcsname{0.72}
\expandafter\xdef\csname used_features_ratio_4\endcsname{0.72}
\expandafter\xdef\csname used_features_ratio_3\endcsname{0.76}
\expandafter\xdef\csname used_features_ratio_2\endcsname{0.76}
\expandafter\xdef\csname used_features_ratio_1\endcsname{0.85}
\expandafter\xdef\csname used_features_ratio_0\endcsname{1.00}

